REALM-Bench: A Benchmark for Evaluating Multi-Agent Systems on Real-world, Dynamic Planning and Scheduling Tasks

This benchmark suite provides a comprehensive evaluation framework for assessing both individual LLMs and multi-agent systems in Real-world planning and scheduling scenarios. The suite encompasses 14 designed planning and scheduling problems that progress from basic to highly complex, incorporating key aspects such as multi-agent coordination, inter-agent dependencies, and dynamic environmental disruptions. Each problem can be scaled along three dimensions: the number of parallel planning threads, the complexity of inter-dependencies, and the frequency of unexpected disruptions requiring Real-time adaptation. The benchmark includes 14 detailed problem specifications, 15 comparison methods including Random, LPT, SPT, STPT, MPSR, DRL-Liu, GP, GEP, LSO, SPT/TWKR, DRL-Chen, DRL-Zhang, 2+ evaluation metrics, and baseline implementations using 3+ LLMs including GPT-4o, Claude-3.7, DeepSeek-R1, and 4 contemporary frameworks including LangGraph, AutoGen, CrewAI, and Swarm, enabling rigorous testing of both single-agent and multi-agent planning capabilities. Through standardized evaluation criteria and scalable complexity, this benchmark aims to be opened to public, and drive progress in developing more adaptable, robust, and scalable AI planning systems for Real-world applications.

==> PoblemSupplyChain.tex <==
\begin{table*}[th!]
\caption{Summary of the Data Center Construction Problem Statement}
\label{tab:ProblemSupplyChain}
\vspace{-,1in}
\centering
\resizebox{\textwidth}{!}{%
\footnotesize
\begin{tabular}{|p{3.3cm}|p{13.6cm}|}
\hline
\textbf{Component} & \textbf{Details} \\
\hline
\multicolumn{2}{|l|}{\textbf{GPU Procurement \& Shipments}} \\
\hline
Total GPU Target & 100,000 units \\
\hline
Vendors & 
\begin{tabular}[c]{@{}l@{}}
\textbf{NVIDIA:} \$15k/unit, 200k units/quarter capacity, 20\% maintenance risk (of unit price over 1 year)\\
\textbf{AMD:} \$10k/unit, 150k units/quarter capacity,  50\% maintenance risk (of unit price over 1 year)
\end{tabular} \\
\hline
Order Timing & All orders placed on Day 1 \\
\hline
Shipment Schedule & Quarterly shipments; e.g., a 600,000 unit order results in 3 shipments of 200,000 units at the end of Q1, Q2, and Q3 \\
\hline
Payment Terms & 50\% deposit at order (day 1), 50\% at delivery (each quarter) \\
\hline
\multicolumn{2}{|l|}{\textbf{Natural Disaster Impacts}} \\
\hline
Risk Probabilities & Earthquake: 10\% per quarter; Typhoon: 10\% per quarter (assessed over entire project) \\
\hline
Delay Impact & Cascading 1-month delay on all subsequent shipments if a disaster occurs in a quarter \\
\hline
Cost Impact & 30\% price increase applied only to the affected quarter’s shipment \\
\hline
Shipment Expedition Impact & Expedite one shipment by 1 month and all subsequent shipments are moved up by 1 month (lock stepped) \\
\hline
\multicolumn{2}{|l|}{\textbf{Cluster Construction \& Infrastructure}} \\
\hline
Cluster Definition & Each cluster requires 50,000 GPUs; clusters can be built concurrently once required GPUs are delivered \\
\hline
\multicolumn{2}{|l|}{\textbf{Networking Infrastructure (per cluster)}} \\
\hline
Duration & 1 months \\
\hline
Cost & \$25 million \\
\hline
Dependencies & Can begin only after GPUs have arrived, power is ready, and cooling is operational \\
\hline
\multicolumn{2}{|l|}{\textbf{Power \& Cooling (per cluster)}} \\
\hline
Requirements & Power: 150 MW; Cooling: 1M gallons/day \\
\hline
Lead Time Options & 
\begin{tabular}[c]{@{}l@{}}Regular: 2 months at \$30M per cluster\\ Expedited: 1 months at \$75M per cluster (150\% cost premium)\end{tabular} \\
\hline
\multicolumn{2}{|l|}{\textbf{Testing \& Certification (per cluster)}} \\
\hline
Normal Process & 2 months, \$15 million \\
\hline
Expedited Process & 1 month, \$45 million (150\% cost premium) \\
\hline
Expedition Options & Expedite power/cooling, networking (50\% time reduction, 150\% cost premium), and testing independently per cluster \\
\hline
\multicolumn{2}{|l|}{\textbf{Business Impact of Delays}} \\
\hline
Delay Costs & \$50 million lost revenue + \$10 million additional operating costs per month of delay \\
\hline
\multicolumn{2}{|l|}{\textbf{Overall Objective}} \\
\hline
Objective & Minimize the end-to-end construction cost (procurement, construction, maintenance, delay costs, expedition premiums) while meeting the 15-month deadline. If the 15-month not met, adding delay costs \\
\hline
\end{tabular}
}
\vspace{-.1in}
\end{table*}

